Cartoon Approximation with $\alpha$-Curvelets

It is well-known that curvelets provide optimal approximations for so-called cartoon images which are defined as piecewise $C^2$-functions, separated by a $C^2$ singularity curve. In this paper, we consider the more general case of piecewise $C^\beta$-functions, separated by a $C^\beta$ singularity curve for $\beta \in (1,2]$. We first prove a benchmark result for the possibly achievable best $N$-term approximation rate for this more general signal model. Then we introduce what we call $\alpha$-curvelets, which are systems that interpolate between wavelet systems on the one hand ($\alpha = 1$) and curvelet systems on the other hand ($\alpha = \frac12$). Our main result states that those frames achieve this optimal rate for $\alpha = \frac{1}{\beta}$, up to $\log$-factors.

==> abstract <==
It is well-known that curvelets provide optimal approximations for so-called cartoon images
which are defined as piecewise $C^2$-functions, separated by a $C^2$ singularity curve. In this
paper, we consider the more general case of piecewise $C^\beta$-functions, separated by a $C^\beta$
singularity curve for $\beta \in (1,2]$. We first prove a benchmark result for the possibly achievable
best $N$-term approximation rate for this more general signal model. Then we introduce what we call
$\alpha$-curvelets, which are systems that interpolate between wavelet systems on the one hand
($\alpha = 1$) and curvelet systems on the other hand ($\alpha = \frac12$). Our main result
states that those frames achieve this optimal rate for $\alpha = \frac{1}{\beta}$, up to $\log$-factors.

